ImageReward: Learning and Evaluating Human Preferences for Text-to-Image Generation

We present a comprehensive solution to learn and improve text-to-image models from human preference feedback. To begin with, we build ImageReward -- the first general-purpose text-to-image human preference reward model -- to effectively encode human preferences. Its training is based on our systematic annotation pipeline including rating and ranking, which collects 137k expert comparisons to date. In human evaluation, ImageReward outperforms existing scoring models and metrics, making it a promising automatic metric for evaluating text-to-image synthesis. On top of it, we propose Reward Feedback Learning (ReFL), a direct tuning algorithm to optimize diffusion models against a scorer. Both automatic and human evaluation support ReFL's advantages over compared methods. All code and datasets are provided at \url{https://github.com/THUDM/ImageReward}.

==> 8_limitation.tex <==
\section*{Limitations}
In this section, we discuss some limitations we realize during the development of \model.

\vpara{Annotation scale, diversity, and quality.} Although our annotation data has reached up to about 9k prompts and 137k pairs of expert comparisons, the larger scale of the annotation dataset is still needed for better RM training. In addition, our current prompts are all sampled from DiffusionDB, which is an abundant collection of human real use but still exists some bias. 
% \hide{For example, we find that many of these prompts use very complex and decorative diction such as "cyberpunk face, fantasy, intricate, elegant, highly detailed", or with a very strange imagination such as "kawaii portrait Aurora (white haired Singer Ferret) seen eating of the strangling network of yellowcake aero chrome and milky Fruit", etc. }
Despite these prompts may close to many real cases, biases exist since the real application when people use the text-to-image model are far beyond trying strange prompts. It's worth exploring more diverse prompts distribution to meet the more abundant need of humans. Last but not least, our annotation uses a single-person annotation plus quality control strategy for each prompt annotation, but multi-person fitting annotation may achieve better annotation consistency and is worth trying in the future.

\vpara{RM training techniques.} As we mentioned in Section~\ref{RM_training}, overfitting dose affects the RM training, and fixing part of transformer layers helps a lot. Nevertheless, we speculate that more advanced techniques (e.g., parameter-efficient tuning~\cite{li2021prefix,liu2021gpt,lester2021power,liu2021p}) could be helpful for the problem.
On the other hand, since BLIP improves over CLIP substantially in \model training, we also expect a stronger and larger text-image backbone model may contribute to additional gains.

\vpara{Using RM to improve generative models.}
% Though posthoc selection is useful for enhancing image quality, we hope \model to fundamentally improve existing text-to-image generative models via serving as a real RM in RLHF.
% However, RLHF in natural language processing is applied to transformer-based generative models. In text-to-image synthesis, the dominant diffusion-based models seem not naturally conformable to RLHF's existing paradigm.
% Despite the recent~\cite{lee2023aligning}'s attempt to leverage reward-witnessed training in a closed domain, the vanilla RLHF is proved more data-efficient, effective, and generalizable in real environments.
% We hope to closely collaborate with the research community to solve the challenge in the future.
Though we have proposed ReFL as an effective method to utilize human preference scorers' feedback to optimize LDMs, it remains an approximation of original RLHF algorithms and could be improved fundamentally.
It is necessary to develop corresponding unbiased and efficient feedback learning algorithms with solid theory groundings to allow better human alignment.


\section*{Broader Impact}

The aim of this paper is to introduce human preference feedback to improve text-to-image generation, which will help image generation to better match the needs of human life and to conform to social norms. Fine-tuning the model with human feedback helps to avoid researchers from over-relying on various types of data with copyright issues for training, and can instead directly improve performance with reward model feedback. A downside is that the preferences of a single reward model are not representative of the multiplicity of human aesthetics, and we can address this by training a variety of reward models and limiting the use of individual reward models. We believe that these benefits outweigh the drawbacks.

==> Tables/ablation_result_table.tex <==
\begin{table}[t]
  \caption{Ablation study for different backbones used in \model. The architecture is  all an MLP added on the output of pre-trained backbone transformer layers (ViT-L for image encoder, 12-layers transformer for text encoder).}
  \vspace{0.5mm}
  \label{ablation_result}
  \centering
  \small
  \begin{tabular}{c|c|c|ccc|ccc}
    \toprule
      \multirow{2}*{Backbone} & Training & Preference & \multicolumn{3}{c|}{Recall} & \multicolumn{3}{c}{Filter} \\
      ~ & Set Size & Acc. & @1 & @2 & @4 & @1 & @2 & @4 \\
    \midrule
      \multirow{2}*{CLIP} & 4k & 61.87 & 38.54 & 57.95 & 81.67 & 46.90 & 63.34 & 85.71 \\
       & 8k & 62.98 & 38.01 & 57.95 & 84.91 & 47.71 & 65.77 & 85.71 \\
    \midrule
      \multirow{4}*{BLIP} & 1k & 63.07 & 34.50 & 55.80 & 85.44 & 42.05 & 65.23 & 84.37 \\
       & 2k & 63.18 & 39.35 & 62.26 & 88.95 & 46.36 & 67.92 & 88.41 \\
       & 4k & 64.71 & \textbf{41.51} & 62.53 & 88.68 & 46.90 & \textbf{70.62} & \textbf{89.49} \\
       & 8k & \textbf{65.14} & 39.62 & \textbf{63.07} & \textbf{90.57} & \textbf{49.06} & \textbf{70.62} & 88.95 \\
    \bottomrule
  \end{tabular}
  \vspace{-4mm}
\end{table}

==> Tables/agreement_table.tex <==
\begin{table}[h]
    \vspace{-2mm}
    \caption{Agreement between different annotators, researchers, and models. The standard deviation is recorded after the $\pm$ in the table. Especially, "annotator ensemble" means, for each pair of images, we use the image considered better by most people as the better one. When comparing an annotator and the ensemble, the annotator is excluded from the ensemble.}
    % For each prompt, several images are generated by the model, and all images are ranked by the annotator or the machine. Therefore, each pair of images either rank equally, or there is a better one. When calculating agreement between two annotators, for each pair of images, if two annotators choose the same image as the better one, this pair is counted as a "similar pair"; if one of the annotators thinks the two images rank the same, this pair will be ignored. The final agreement between two annotators is the count of "similar pairs" divided by the count of all image pairs. When calculating the agreement between two groups, if there are multiple annotators in the group, there will exist multiple agreements between annotators. Then we take the average of all the agreements as the final agreement, and the standard deviation is recorded after the $\pm$ in the table. Especially, "annotator ensemble" means, for each pair of images, we use the image considered better by most people as the better one.
    \small
    \vspace{1mm}
    \label{agree_exclude}
    \centering
    \renewcommand\tabcolsep{1.5pt}
    % \renewcommand\arraystretch{1.2}
    \begin{tabular}{c|ccc|cccc}
        \toprule
        ~ & researcher & annotator & \makecell[c]{annotator\\ensemble} & \makecell[c]{CLIP\\Score} & Aesthetic & \makecell[c]{BLIP\\Score} & Ours \\
        \midrule
        researcher & \makecell[c]{71.2\% \\ \scriptsize{$\pm$ 11.1\%} } & \makecell[c]{65.3\% \\ \scriptsize{$\pm$ 8.5\%} } & \makecell[c]{73.4\% \\ \scriptsize{$\pm$ 6.2\%} } & \makecell[c]{57.8\% \\ \scriptsize{$\pm$ 3.6\%} } & \makecell[c]{55.6\% \\ \scriptsize{$\pm$ 3.1\%} } & \makecell[c]{57.0\% \\ \scriptsize{$\pm$ 3.0\%} } & \textbf{\makecell[c]{64.5\% \\ \scriptsize{$\pm$ 2.5\%} }} \\
        \midrule
        annotator & \makecell[c]{65.3\% \\ \scriptsize{$\pm$ 8.5\%} } & \makecell[c]{65.3\% \\ \scriptsize{$\pm$ 5.6\%} } & \makecell[c]{53.9\% \\ \scriptsize{$\pm$ 5.8\%} } & \makecell[c]{54.3\% \\ \scriptsize{$\pm$ 3.2\%} } & \makecell[c]{55.9\% \\ \scriptsize{$\pm$ 3.1\%} } & \makecell[c]{57.4\% \\ \scriptsize{$\pm$ 2.7\%} } & \textbf{\makecell[c]{65.3\% \\ \scriptsize{$\pm$ 3.7\%} }} \\
        \midrule
        \makecell[c]{annotator\\ensemble} & \makecell[c]{73.4\% \\ \scriptsize{$\pm$ 6.2\%} } & \makecell[c]{53.9\% \\ \scriptsize{$\pm$ 5.8\%} } & - & \makecell[c]{54.4\% \\ \scriptsize{$\pm$ 21.1\%} } & \makecell[c]{57.5\% \\ \scriptsize{$\pm$ 15.9\%} } & \makecell[c]{62.0\% \\ \scriptsize{$\pm$ 16.1\%} } & \textbf{\makecell[c]{70.5\% \\ \scriptsize{$\pm$ 18.6\%} }} \\
        \bottomrule
    \end{tabular}
\end{table}

==> Tables/denoising_rate.tex <==
\begin{table}[h]
    \vspace{-2mm}
    \caption{TBD}
    \vspace{1mm}
    \label{tab:denoising}
    \centering
    \renewcommand\tabcolsep{1.5pt}
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
        \toprule
        Denoising Step & 5 & 10 & 15 & 20 & 25 & 30 & 35 & 40 \\
        \midrule
        Spearman $\rho$ & 0.0623 & 0.1073 & 0.1180 & 0.2980 & 0.5519 & 0.7884 & 0.9191 & 1.0000  \\
        \bottomrule
    \end{tabular}
\end{table}

==> Tables/fine_copy.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{Comparison between different reward feedback or fine-tune methods. Human evaluation include 5 annotators to rate and rank all generated images, which is the same process as annotation. All ratings are seven-point Likert scale.}
    \vspace{1mm}
    \label{tab:finetune_table}
    \renewcommand\tabcolsep{3.5pt}
    \begin{tabular}{lcccc|cccc}
        \toprule
        \multirow{3}{*}{Methods} & \multicolumn{4}{c}{Real User Prompts} & \multicolumn{4}{|c}{Real User Prompts} \\ 
        \cmidrule(l){2-5} \cmidrule(l){6-9} 
        & \multicolumn{3}{c}{Human Eval.} & Image & \multicolumn{3}{|c}{Human Eval.} & Image \\ 
        \cmidrule(l){2-4}  \cmidrule(l){6-8} 
        & Align. & Fidelity & Overall & Reward & rank-mean & rank-mrr & Overall & Reward \\ 
        \midrule
        SD v1.4 (baseline)\cite{rombach2022high} & 4.41 & 4.64 & 4.59 & 0.1058 & 2.62 & 0.51 & 20.7 & 0.1859 \\
        \midrule
        BoN (N=4) & \textbf{4.74} & \textbf{5.00} & \textbf{4.82} & 0.8228 & 2.20 & 0.60 & 20.7 & 0.7686 \\
        BoN (N=16) & 4.70 & 4.90 & 4.76 & 1.1418 & \textbf{2.18} & \textbf{0.61} & 20.7 & 1.1659 \\
        BoN (N=64) & 4.65 & 4.92 & 4.74 & \textbf{1.3374} & 2.25 & 0.59 & 20.7 & \textbf{1.4098} \\
        \midrule
        Dataset Filtering\cite{wu2023better} & \textbf{4.24} & \textbf{4.55} & \textbf{4.34} & 0.2000 & \textbf{2.80} & \textbf{0.45} & 20.7 & 0.3289 \\
        Reward Weighted\cite{lee2023aligning} & 3.99 & 4.47 & 4.12 & 0.2475 & 3.14 & 0.38 & 20.7 & 0.3059 \\
        RAHF\cite{dong2023raft} (iteration=1) & 4.22 & 4.63 & 4.30 & 0.3571 & 2.81 & 0.44 & 20.7 & \textbf{0.4594} \\
        RAHF (iteration=2) & 3.87 & 4.42 & 3.89 & 0.3654 & 3.33 & 0.36 & 20.7 & 0.3663 \\
        RAHF (iteration=3) & 3.17 & 3.88 & 3.20 & 0.1422 & 4.06 & 0.28 & 20.7 & 0.2061 \\
        \midrule
        \textbf{ReFL (Ours)} & 4.18 & 4.51 & 4.12 & \textbf{0.6955} & 2.95 & 0.43 & 20.7 & 0.2635 \\
        \bottomrule
    \end{tabular}
    \vspace{-5mm}
\end{table}

